A Suite of Metrics for Calculating the Most Significant Security Relevant Software Flaw Types

The Common Weakness Enumeration (CWE) is a prominent list of software weakness types. This list is used by vulnerability databases to describe the underlying security flaws within analyzed vulnerabilities. This linkage opens the possibility of using the analysis of software vulnerabilities to identify the most significant weaknesses that enable those vulnerabilities. We accomplish this through creating mashup views combining CWE weakness taxonomies with vulnerability analysis data. The resulting graphs have CWEs as nodes, edges derived from multiple CWE taxonomies, and nodes adorned with vulnerability analysis information (propagated from children to parents). Using these graphs, we develop a suite of metrics to identify the most significant weakness types (using the perspectives of frequency, impact, exploitability, and overall severity).

==> Keywords.tex <==
Metrics, Software flaws, Vulnerabilities

==> TopTables.tex <==
\begin{table*}[]
\centering
\caption{Top CWE Classes Relative to Normalized Frequency}
\begin{tabular}{lllll}
1 & CWE-20 & Improper Input Validation & 1.00 \\
2 & CWE-119 & Improper Restriction of Operations within the Bounds of a Memory Buffer & 0.72 \\
3 & CWE-116 & Improper Encoding or Escaping of Output & 0.61 \\
4 & CWE-74 & Improper Neutralization of Special Elements in Output Used by a Downstream Component ('Injection') & 0.61 \\
5 & CWE-668 & Exposure of Resource to Wrong Sphere & 0.58 \\
6 & CWE-200 & Information Exposure & 0.27 \\
7 & CWE-672 & Operation on a Resource after Expiration or Release & 0.22 \\
8 & CWE-610 & Externally Controlled Reference to a Resource in Another Sphere & 0.18 \\
9 & CWE-287 & Improper Authentication & 0.15 \\
10 & CWE-345 & Insufficient Verification of Data Authenticity & 0.12 \\
11 & CWE-706 & Use of Incorrectly-Resolved Name or Reference & 0.09 \\
12 & CWE-754 & Improper Check for Unusual or Exceptional Conditions & 0.07 \\
13 & CWE-400 & Uncontrolled Resource Consumption & 0.07 \\
14 & CWE-732 & Incorrect Permission Assignment for Critical Resource & 0.07 \\
15 & CWE-269 & Improper Privilege Management & 0.06 \\
\begin{comment}
16 & CWE-682 & Incorrect Calculation & 0.06 \\
17 & CWE-669 & Incorrect Resource Transfer Between Spheres & 0.05 \\
18 & CWE-913 & Improper Control of Dynamically-Managed Code Resources & 0.05 \\
19 & CWE-330 & Use of Insufficiently Random Values & 0.03 \\
20 & CWE-863 & Incorrect Authorization & 0.02 \\
\end{comment}
\end{tabular}
\label{Tab:ClassesFrequency}
\end{table*}

\begin{table*}[]
\centering
\caption{Top CWE Classes Relative to Mean Exploitability}
\begin{tabular}{lllll}
1 & CWE-436 & Interpretation Conflict & 3.64 \\
2 & CWE-400 & Uncontrolled Resource Consumption & 3.35 \\
3 & CWE-330 & Use of Insufficiently Random Values & 3.28 \\
4 & CWE-834 & Excessive Iteration & 3.27 \\
5 & CWE-404 & Improper Resource Shutdown or Release & 3.21 \\
6 & CWE-670 & Always-Incorrect Control Flow Implementation & 3.16 \\
7 & CWE-706 & Use of Incorrectly-Resolved Name or Reference & 3.11 \\
8 & CWE-287 & Improper Authentication & 3.10 \\
9 & CWE-755 & Improper Handling of Exceptional Conditions & 3.10 \\
10 & CWE-326 & Inadequate Encryption Strength & 3.10 \\
11 & CWE-913 & Improper Control of Dynamically-Managed Code Resources & 3.09 \\
12 & CWE-704 & Incorrect Type Conversion or Cast & 3.07 \\
13 & CWE-327 & Use of a Broken or Risky Cryptographic Algorithm & 3.02 \\
14 & CWE-669 & Incorrect Resource Transfer Between Spheres & 2.92 \\
15 & CWE-674 & Uncontrolled Recursion & 2.90 \\
\begin{comment}
16 & CWE-754 & Improper Check for Unusual or Exceptional Conditions & 2.88 \\
17 & CWE-610 & Externally Controlled Reference to a Resource in Another Sphere & 2.85 \\
18 & CWE-863 & Incorrect Authorization & 2.83 \\
19 & CWE-665 & Improper Initialization & 2.82 \\
20 & CWE-200 & Information Exposure & 2.80 \\
\end{comment}
\end{tabular}
\label{Tab:ClassesExploitability}
\end{table*}

\begin{table*}[]
\centering
\caption{Top CWE Classes Relative to Mean Impact}
\begin{tabular}{lllll}
1 & CWE-913 & Improper Control of Dynamically-Managed Code Resources & 5.65 \\
2 & CWE-704 & Incorrect Type Conversion or Cast & 5.59 \\
3 & CWE-269 & Improper Privilege Management & 5.47 \\
4 & CWE-669 & Incorrect Resource Transfer Between Spheres & 5.36 \\
5 & CWE-362 & Concurrent Execution using Shared Resource with Improper Synchronization ('Race Condition') & 5.19 \\
6 & CWE-119 & Improper Restriction of Operations within the Bounds of a Memory Buffer & 5.17 \\
7 & CWE-672 & Operation on a Resource after Expiration or Release & 5.16 \\
8 & CWE-330 & Use of Insufficiently Random Values & 5.07 \\
9 & CWE-345 & Insufficient Verification of Data Authenticity & 4.94 \\
10 & CWE-682 & Incorrect Calculation & 4.91 \\
11 & CWE-287 & Improper Authentication & 4.71 \\
12 & CWE-610 & Externally Controlled Reference to a Resource in Another Sphere & 4.51 \\
13 & CWE-732 & Incorrect Permission Assignment for Critical Resource & 4.27 \\
14 & CWE-326 & Inadequate Encryption Strength & 4.13 \\
15 & CWE-754 & Improper Check for Unusual or Exceptional Conditions & 4.10 \\
\begin{comment}
16 & CWE-706 & Use of Incorrectly-Resolved Name or Reference & 4.03 \\
17 & CWE-20 & Improper Input Validation & 3.95 \\
18 & CWE-863 & Incorrect Authorization & 3.90 \\
19 & CWE-665 & Improper Initialization & 3.87 \\
20 & CWE-668 & Exposure of Resource to Wrong Sphere & 3.85 \\
\end{comment}
\end{tabular}
\label{Tab:ClassesImpact}
\end{table*}

\begin{comment}
\begin{table*}[]
\centering
\caption{Top CWE Classes Relative to Mean CVSS Score}
\begin{tabular}{lllll}
1 & CWE-913 & Improper Control of Dynamically-Managed Code Resources & 8.80 \\
2 & CWE-704 & Incorrect Type Conversion or Cast & 8.73 \\
3 & CWE-330 & Use of Insufficiently Random Values & 8.39 \\
4 & CWE-669 & Incorrect Resource Transfer Between Spheres & 8.34 \\
5 & CWE-119 & Improper Restriction of Operations within the Bounds of a Memory Buffer & 7.99 \\
6 & CWE-672 & Operation on a Resource after Expiration or Release & 7.99 \\
7 & CWE-287 & Improper Authentication & 7.86 \\
8 & CWE-682 & Incorrect Calculation & 7.77 \\
9 & CWE-345 & Insufficient Verification of Data Authenticity & 7.77 \\
10 & CWE-269 & Improper Privilege Management & 7.76 \\
11 & CWE-610 & Externally Controlled Reference to a Resource in Another Sphere & 7.51 \\
12 & CWE-326 & Inadequate Encryption Strength & 7.27 \\
13 & CWE-706 & Use of Incorrectly-Resolved Name or Reference & 7.20 \\
14 & CWE-400 & Uncontrolled Resource Consumption & 7.05 \\
15 & CWE-404 & Improper Resource Shutdown or Release & 7.05 \\
16 & CWE-754 & Improper Check for Unusual or Exceptional Conditions & 7.04 \\
17 & CWE-20 & Improper Input Validation & 6.99 \\
18 & CWE-670 & Always-Incorrect Control Flow Implementation & 6.89 \\
19 & CWE-834 & Excessive Iteration & 6.83 \\
20 & CWE-116 & Improper Encoding or Escaping of Output & 6.82 \\
\end{tabular}
\label{Tab:ClassesCVSS}
\end{table*}
\end{comment}

\begin{table*}[]
\centering
\caption{Top CWEs Relative to Normalized Frequency for Bases, Variants, and Compounds}
\begin{tabular}{lllll}
1 & CWE-79 & Improper Neutralization of Input During Web Page Generation ('Cross-site Scripting') & 1.00 \\
2 & CWE-125 & Out-of-bounds Read & 0.45 \\
3 & CWE-416 & Use After Free & 0.28 \\
4 & CWE-346 & Origin Validation Error & 0.27 \\
5 & CWE-787 & Out-of-bounds Write & 0.27 \\
6 & CWE-89 & Improper Neutralization of Special Elements used in an SQL Command ('SQL Injection') & 0.26 \\
7 & CWE-613 & Insufficient Session Expiration & 0.26 \\
8 & CWE-352 & Cross-Site Request Forgery (CSRF) & 0.25 \\
9 & CWE-22 & Improper Limitation of a Pathname to a Restricted Directory ('Path Traversal') & 0.21 \\
10 & CWE-476 & NULL Pointer Dereference & 0.16 \\
11 & CWE-434 & Unrestricted Upload of File with Dangerous Type & 0.12 \\
12 & CWE-190 & Integer Overflow or Wraparound & 0.11 \\
13 & CWE-78 & Improper Neutralization of Special Elements used in an OS Command ('OS Command Injection') & 0.10 \\
14 & CWE-120 & Buffer Copy without Checking Size of Input ('Classic Buffer Overflow') & 0.08 \\
15 & CWE-94 & Improper Control of Generation of Code ('Code Injection') & 0.07 \\
\begin{comment}
16 & CWE-611 & Improper Restriction of XML External Entity Reference & 0.07 \\
17 & CWE-601 & URL Redirection to Untrusted Site ('Open Redirect') & 0.06 \\
18 & CWE-798 & Use of Hard-coded Credentials & 0.05 \\
19 & CWE-502 & Deserialization of Untrusted Data & 0.05 \\
20 & CWE-522 & Insufficiently Protected Credentials & 0.05 \\
\end{comment}
\end{tabular}
\label{Tab:BasesFrequency}
\end{table*}

\begin{table*}[]
\centering
\caption{Top CWEs Relative to Mean Exploitability for Bases, Variants, and Compounds}
\begin{tabular}{lllll}
1 & CWE-131 & Incorrect Calculation of Buffer Size & 3.90 \\
2 & CWE-273 & Improper Check for Dropped Privileges & 3.90 \\
3 & CWE-838 & Inappropriate Encoding for Output Context & 3.90 \\
4 & CWE-331 & Insufficient Entropy & 3.90 \\
5 & CWE-307 & Improper Restriction of Excessive Authentication Attempts & 3.76 \\
6 & CWE-521 & Weak Password Requirements & 3.72 \\
7 & CWE-444 & Inconsistent Interpretation of HTTP Requests ('HTTP Request Smuggling') & 3.61 \\
8 & CWE-306 & Missing Authentication for Critical Function & 3.54 \\
9 & CWE-565 & Reliance on Cookies without Validation and Integrity Checking & 3.53 \\
10 & CWE-209 & Information Exposure Through an Error Message & 3.53 \\
11 & CWE-88 & Improper Neutralization of Argument Delimiters in a Command ('Argument Injection') & 3.35 \\
12 & CWE-470 & Use of Externally-Controlled Input to Select Classes or Code ('Unsafe Reflection') & 3.35 \\
13 & CWE-640 & Weak Password Recovery Mechanism for Forgotten Password & 3.34 \\
14 & CWE-502 & Deserialization of Untrusted Data & 3.33 \\
15 & CWE-89 & Improper Neutralization of Special Elements used in an SQL Command ('SQL Injection') & 3.30 \\
\begin{comment}
16 & CWE-798 & Use of Hard-coded Credentials & 3.29 \\
17 & CWE-835 & Loop with Unreachable Exit Condition ('Infinite Loop') & 3.27 \\
18 & CWE-203 & Information Exposure Through Discrepancy & 3.26 \\
19 & CWE-918 & Server-Side Request Forgery (SSRF) & 3.26 \\
20 & CWE-22 & Improper Limitation of a Pathname to a Restricted Directory ('Path Traversal') & 3.23 \\
\end{comment}
\end{tabular}
\label{Tab:BasesExploitability}
\end{table*}

\begin{table*}[]
\centering
\caption{Top CWEs Relative to Mean Impact for Bases, Variants, and Compounds}
\begin{tabular}{lllll}
1 & CWE-78 & Improper Neutralization of Special Elements used in an OS Command ('OS Command Injection') & 5.90 \\
2 & CWE-131 & Incorrect Calculation of Buffer Size & 5.90 \\
3 & CWE-273 & Improper Check for Dropped Privileges & 5.90 \\
4 & CWE-838 & Inappropriate Encoding for Output Context & 5.90 \\
5 & CWE-428 & Unquoted Search Path or Element & 5.90 \\
6 & CWE-426 & Untrusted Search Path & 5.80 \\
7 & CWE-94 & Improper Control of Generation of Code ('Code Injection') & 5.71 \\
8 & CWE-129 & Improper Validation of Array Index & 5.66 \\
9 & CWE-502 & Deserialization of Untrusted Data & 5.65 \\
10 & CWE-787 & Out-of-bounds Write & 5.61 \\
11 & CWE-89 & Improper Neutralization of Special Elements used in an SQL Command ('SQL Injection') & 5.61 \\
12 & CWE-427 & Uncontrolled Search Path Element & 5.55 \\
13 & CWE-120 & Buffer Copy without Checking Size of Input ('Classic Buffer Overflow') & 5.55 \\
14 & CWE-434 & Unrestricted Upload of File with Dangerous Type & 5.46 \\
15 & CWE-798 & Use of Hard-coded Credentials & 5.44 \\
\begin{comment}
16 & CWE-191 & Integer Underflow (Wrap or Wraparound) & 5.44 \\
17 & CWE-843 & Access of Resource Using Incompatible Type ('Type Confusion') & 5.40 \\
18 & CWE-307 & Improper Restriction of Excessive Authentication Attempts & 5.33 \\
19 & CWE-415 & Double Free & 5.32 \\
20 & CWE-416 & Use After Free & 5.25 \\
\end{comment}
\end{tabular}
\label{Tab:BasesImpact}
\end{table*}

\begin{comment}
\begin{table*}[]
\centering
\caption{Top CWEs Relative to Mean CVSS Score for Bases, Variants, and Compounds}
\begin{tabular}{lllll}
1 & CWE-131 & Incorrect Calculation of Buffer Size & 9.80 \\
2 & CWE-273 & Improper Check for Dropped Privileges & 9.80 \\
3 & CWE-838 & Inappropriate Encoding for Output Context & 9.80 \\
4 & CWE-307 & Improper Restriction of Excessive Authentication Attempts & 9.10 \\
5 & CWE-502 & Deserialization of Untrusted Data & 9.02 \\
6 & CWE-89 & Improper Neutralization of Special Elements used in an SQL Command ('SQL Injection') & 8.95 \\
7 & CWE-798 & Use of Hard-coded Credentials & 8.78 \\
8 & CWE-94 & Improper Control of Generation of Code ('Code Injection') & 8.70 \\
9 & CWE-521 & Weak Password Requirements & 8.68 \\
10 & CWE-640 & Weak Password Recovery Mechanism for Forgotten Password & 8.63 \\
11 & CWE-78 & Improper Neutralization of Special Elements used in an OS Command ('OS Command Injection') & 8.55 \\
12 & CWE-191 & Integer Underflow (Wrap or Wraparound) & 8.49 \\
13 & CWE-120 & Buffer Copy without Checking Size of Input ('Classic Buffer Overflow') & 8.48 \\
14 & CWE-434 & Unrestricted Upload of File with Dangerous Type & 8.46 \\
15 & CWE-787 & Out-of-bounds Write & 8.41 \\
16 & CWE-129 & Improper Validation of Array Index & 8.40 \\
17 & CWE-88 & Improper Neutralization of Argument Delimiters in a Command ('Argument Injection') & 8.25 \\
18 & CWE-415 & Double Free & 8.13 \\
19 & CWE-91 & XML Injection (aka Blind XPath Injection) & 8.07 \\
20 & CWE-416 & Use After Free & 8.06 \\
\end{tabular}
\label{Tab:BasesCVSS}
\end{table*}
\end{comment}
